Scaling up Dynamic Edge Partition Models via Stochastic Gradient MCMC

The edge partition model (EPM) is a generative model for extracting an overlapping community structure from static graph-structured data. In the EPM, the gamma process (GaP) prior is adopted to infer the appropriate number of latent communities, and each vertex is endowed with a gamma distributed positive memberships vector. Despite having many attractive properties, inference in the EPM is typically performed using Markov chain Monte Carlo (MCMC) methods that prevent it from being applied to massive network data. In this paper, we generalize the EPM to account for dynamic enviroment by representing each vertex with a positive memberships vector constructed using Dirichlet prior specification, and capturing the time-evolving behaviour of vertices via a Dirichlet Markov chain construction. A simple-to-implement Gibbs sampler is proposed to perform posterior computation using Negative- Binomial augmentation technique. For large network data, we propose a stochastic gradient Markov chain Monte Carlo (SG-MCMC) algorithm for scalable inference in the proposed model. The experimental results show that the novel methods achieve competitive performance in terms of link prediction, while being much faster.

==> LNME.tex <==
\begin{tikzpicture}

  % Define nodes
  \node[latent]                  (bmn1) {$x_{nm}^{\scriptscriptstyle(1)}$};
  \node[latent, right=of bmn1, xshift=-0.65cm] (bmn2) {$x_{nm}^{\scriptscriptstyle(2)}$};
  \node[draw=none,right=of bmn2, xshift=-0.65cm]  (bmn3) {$\cdots$};
  \node[latent, right=of bmn3, xshift=-0.65cm] (bmnt)  {$x_{nm}^{\scriptscriptstyle(T)}$};
  % \node[draw=none,right=of bmnt, xshift=-0.65cm]  (bmnT) {$\cdots$};
  
  \node[obs, below= of bmn1, yshift=0.45cm]                  (amn1) {$b_{nm}^{\scriptscriptstyle(1)}$};
  \node[obs, below=of bmn2, , yshift=0.45cm] (amn2) {$b_{nm}^{\scriptscriptstyle(2)}$};
 \node[draw=none,below=of bmn3, yshift=0cm]  (amn3) {$\cdots$};
  \node[obs, below=of bmnt, yshift=0.45cm] (amnt)  {$b_{nm}^{\scriptscriptstyle(T)}$};
  % \node[draw=none,below=of bmnT, yshift=0cm]  (amnT) {$\cdots$};

 
  \node[latent, above=of bmn1, xshift=0cm, yshift=-0.6cm]  (phi_nm_1) {$\phi_{nk}^{(1)}$};
  \node[latent, above=of bmn2, xshift=0cm, yshift=-0.6cm]  (phi_nm_2) {$\phi_{nk}^{(2)}$};
   \node[draw=none,above=of bmn3]  (phi_nm_3) {$\cdots$};
  \node[latent, above=of bmnt, xshift=0cm, yshift=-0.5cm]  (phi_nm_t) {$\phi_{nk}^{(T)}$};
  % \node[draw=none,above=of bmnT]  (phi_nm_T) {$\cdots$};
   \node[latent, left=of phi_nm_1, xshift=0.65cm]  (phi_nm_0) {$\phi_{nk}^{(0)}$};
  \node[legend_isps, left=of phi_nm_0, yshift=-0.5cm,xshift=0.75cm](g0) {$g_0$};
  \node[legend_isps, left=of phi_nm_0, yshift= 0.5cm,xshift=0.75cm](h0) {$h_0$};
  
  \node[legend_isps, above=of phi_nm_0, yshift=-0.465cm,xshift= -0cm](cn) {$c_n$};
  
  \node[latent, left=of bmn1, xshift=-1.85cm,yshift=-0.85cm]  (lambda) {$\mathbf{\Lambda}$};
  \node[latent, above=of lambda, xshift=-0.625cm]  (xi) {$\xi$};
  \node[latent, above=of lambda, xshift=0.625cm]  (r_k) {$\mathbf{r}$};
  \node[latent, above=of r_k, xshift=0.45cm](gam0) {$\gamma_0$};
  \node[legend_isps, above=of r_k, xshift=-0.315cm](c0) {$c_0$};
  \node[legend_isps, above=of xi, xshift=0.315cm](e0) {$e_0$};
  \node[legend_isps, above=of xi, xshift=-0.315cm](f0) {$f_0$};
  \node[legend_isps, left=of lambda, xshift=0.7cm](beta) {$\beta$};
%  \node[latent, right=2cm of y]            (t) {$\tau$};

  % Connect the nodes
  \edge {bmn1} {amn1};
  \edge {bmn2} {amn2};

  \edge {bmnt} {amnt};

  \edge {g0, h0} {phi_nm_0};
  \edge {phi_nm_0} {phi_nm_1};
   \edge {phi_nm_1} {bmn1, phi_nm_2} ; %
   \edge {phi_nm_2} {bmn2, phi_nm_3} ; 
   % \edge {phi_nm_t} {bmnt, phi_nm_T} ; 
   \edge {xi, r_k} {lambda} ; 
   \edge {gam0} {r_k};
   \edge {c0} {r_k};
   \edge {e0} {xi};
   \edge {f0} {xi};
   \edge {beta} {lambda};
   \draw[->,out=0, in=-152](lambda) to (bmn1);
   \draw[->,out=0, in=-155](lambda) to (bmn2);
   \draw[->,out=0, in=-160](lambda) to (bmnt);
   
   
   \draw[->,out=0, in=120](cn) to (phi_nm_1);
   \draw[->,out=0, in=140](cn) to (phi_nm_2);
   \draw[->,out=0, in=150](cn) to (phi_nm_t);

  % Plates
  \plate {yx} {(phi_nm_0)(phi_nm_1)(phi_nm_2)(phi_nm_3)(phi_nm_t)} {$k = 1,\ldots, K$} ;
  \plate {} {(cn)(phi_nm_0)(phi_nm_1)(phi_nm_2)(phi_nm_3)(phi_nm_t)(bmn1)(bmn2)(bmn3)(bmnt)(amn1)(amn2)(amn3)(amnt)} {$n, m= 1,\ldots, N$} ;

\end{tikzpicture}

==> addpackage.tex <==
\usepackage{amssymb}
%\usepackage{natbib}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amsfonts}
\usepackage{bm} 
\usepackage{graphicx}
\usepackage{rotating}
\usepackage{tikz}
\usetikzlibrary{bayesnet}
\usepackage{tabularx,hhline}
\usepackage{array}
\usepackage{tabulary}
\newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\usepackage{bbm}
\usepackage{array}
\usepackage{multirow}
%\usepackage[colorlinks]{hyperref}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{bbm}
%\usepackage[justification=centering]{caption}
\usepackage{tabularx,booktabs} 
\usepackage{standalone}
\usepackage[acronym,smallcaps,nowarn]{glossaries}
\usepackage{aaai19}  %Required
\usepackage{times}  %Required
\usepackage{helvet}  %Required
\usepackage{courier}  %Required
\usepackage{url}  %Required
\usepackage{graphicx}  %Required
\frenchspacing  %Required
\setlength{\pdfpagewidth}{8.5in}  %Required
\setlength{\pdfpageheight}{11in}  %Required
%PDF Info Is Required:
  \pdfinfo{
/Title (2018 Formatting Instructions for Authors Using LaTeX)
/Author (AAAI Press Staff)}
\setcounter{secnumdepth}{0}  

% ALGORITHMS
 \usepackage{algorithm,algorithmic}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}	
%  \usepackage[algoruled]{algorithm2e}
% \usepackage[noend]{algpseudocode}

\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

\usepackage{hyperref}

%\usepackage[longnamesfirst, authoryear]{natbib}

\usepackage[
  separate-uncertainty = true,
  multi-part-units = repeat
]{siunitx}

==> algo_1.tex <==
\begin{algorithm}[t]
    \DontPrintSemicolon
    \SetAlgoLined
    \SetKwInOut{KwInput}{input}
    \SetKwInOut{KwOutput}{output}
    \KwInput{dynamic relational data $\mathbf{b}^{(1)}, \ldots, \mathbf{b}^{(T)}$}
    Initialize the maximum number of groups $K$, hyperparameters $\beta, \tau, c_0, g_0, h_0$, and parameters $\gamma_0, r_k, \xi, \lambda_{kk'}, \phi_{nk}^{(t)}$\;
    \Repeat{convergence}{
    Sample $x_{mn}^{(t)}$ for non-zero links (Eq.~\ref{eq:lcount})\;
    Sample $x_{mkk'n}^{(t)}$ (Eq.~\ref{eq:la_int_count}) and update\;
    \quad $x_{\cdot kk'\cdot}^{(\cdot)} = \sum_{t}\sum_{m,n\neq m} x_{mkk'n}^{(t)}$\;
    \quad $x_{mk\cdot\cdot}^{(t)} = \sum_{\substack{n\neq m},k'} x_{mkk'n}^{(t)}$\;
    Sample $l_{kk'}$ (Eq.~\ref{eq:l_kk}) and calculate the quantities:\;
    \quad $\theta_{kk'}=\sum_{t, n, m \neq n}\phi_{nk}^{(t)}\phi_{mk'}^{(t)}$,\quad $\tilde{p}_{kk'} = \frac{\theta_{kk'}}{\theta_{kk'} + \beta}$\;
    Sample $r_k$ (Eq.~\ref{eq:r_k}), $\xi$ (Eq.~\ref{eq:xi}), and $\lambda_{kk'}$ (Eq.~\ref{eq:lambda_kk})\;
     %\tcc{backward filtering}
    \For{$t = T$ \emph{to} $1$}{
%    Update $\hat{p}_{k} = \frac{\sum_{k'}\xi^{\delta_{(k,k')}}(r_{k'})^{1-\delta_{(k,k')}}\log(1 - \tilde{p}_{kk'})}{c_0 -\sum_{k'}\xi^{\delta_{(k,k')}}(r_{k'})^{1-\delta_{(k,k')}}\log(1 - \tilde{p}_{kk'})}$\;
    Sample $y_{nk}^{(t)}$ (Eq.~\ref{eq:y}) and update $\varrho_{nk}^{(t)}$ (Eq.~\ref{eq:varrho})\;
    }
    %\tcc{forward sampling}
     \For{$t = 0$ \emph{to} $T$}{
    Sample $\phi_{nk}^{(t)}$ (Eq.~\ref{eq:phi})\;
    }
    Sample $c_0$, $\beta$ (Eq.~\ref{eq:hyper}) and $\gamma_0$~(Eq.~\ref{eq_gam0})\;
    % Sample hyperparameters $\beta$, $\tau, c_0, e_0, f_0, g_0, h_0$\;
%      Draw a single sample $\bz\sim q(\bz;\bv)$\;
%      Compute the auxiliary functions $\hfun\left(\Tcal^{-1}(\bz;\bv);\bv\right)$ and $\ufun\left(\Tcal^{-1}(\bz;\bv);\bv\right)$ (Eq.~\ref{eq:hfun_ufun})\;
%      Estimate $\bg^{\textrm{rep}}$ and $\bg^{\textrm{corr}}$ (Eq.~\ref{eq:grep_gcorr}, estimate the expectation with one sample)\;
%      Compute (analytic) or estimate (Monte Carlo) the gradient of the entropy, $\nabla_{\bv}\ent{q(\bz;\bv)}$\;
%      Compute the noisy gradient $\nabla_{\bv}\Lcal$ (Eq.~\ref{eq:corrected_reparam})\;
%      Set the step-size $\brho^{(i)}$ (Eq.~\ref{eq:step_schedule}) and take a gradient step for $\bv$\; % (Eq.~\ref{eq:v_new})\;
    }
    \KwOutput{posterior mean $\phi_{nk}^{(t)}, r_k, \xi, \lambda_{kk'}, \beta, \gamma_0$}
    \caption{Batch Gibbs Sampling\label{alg:batch-Gibbs}}
\end{algorithm}

==> section_relatedworks.tex <==
\section{Related Work}
% Some related work on graph-structured neural temporal point
% processes (NTPPs) are recapped as we have discussed most NTPPs in the introduction. Additionally, we also discuss those work related to the learning of latent graphs underlying discrete-time observations.
\cite{SN1980,SN03} proposed to capture the non-stationary network dynamics using continuous-time Markov chains. \\
\noindent\textbf{Graph-Structured Temporal Point Processes.}
\cite{PGEM} proposed a proximal graphical event model to infer the relationships among event types, and thus assumes that the occurrence of an event only depends on the occurring of its parents shortly before. 
\cite{GHP} developed a geometric Hawkes process to capture correlations among multiple point processes using graph convolutional neural networks although the inferred graph is {undirected}. 
\cite{THP} developed a graph-structured transformer Hawkes process between multiple point processes. It assumes that each point process is associated with a vertex of a \emph{static} graph, and model the dependency among those point processes by incorporating that graph into the attention module design. \cite{NTPPwithGraph} formulated a graph-structured neural temporal point process (NTPP) by sampling a latent graph using a generator. The model parameters of the graph-structured NTPP and its associated graph, can be simultaneously optimized using an efficient bi-level programming. \cite{ENTPP} recently also developed a variational framework for graph-structured neural point processes by generating a latent graph using intra-type history embeddings. The latent graph is then used to govern the message passing between intra-type embedding to decode the type-wise conditional intensity function. \cite{ijcai2021p469} proposed to learn a static conditional graph  between event types, by incorporating prior knowledge. 
Additionally, \cite{LGPP} proposed to learn the latent graph structure among events via a probabilistic model. \cite{GBTPP} tries to model event propagation using a graph-biased temporal point process, with a graph specified by the following relationships among individuals on social media.  \cite{VAEPP} studied a variational auto-encoder framework for modeling event sequences but haven't consider capturing latent graphs among dimensions. 


\noindent\textbf{Dynamic Latent Graphs behind Time Series.} 
\cite{NRI} developed an variational autoencoder to learn a latent \emph{static} graph among the entities that interact in a physical dynamical system. Following this success, \cite{dNRI} used a sequential latent variable model to infer dynamic latent graphs among the entities from the discrete-time observations. Although \cite{dNRI} and the proposed method both aim to learn dynamic graphs behind multivariate sequential observations, the main differences lie in that our input is \emph{asynchronous} event sequences, for which we need to determine the regularly-spaced sub-intervals, and simultaneously learn a dynamic graph for each sub-interval. An interesting yet challenging direction, is to automatically infer the regularly-spaced time intervals and the corresponding dynamic graph structure, which we leave to future research. 

% For learning and estimating collective dynamics with aggregate data, prior works~\cite{} focused on the modelling of a single Markov model by maximizing aggregate posterior.
%  The recent studies in learning Markov models from aggregate data include~\cite{} with applications on tourist and migration flow analysis.
 
%  Collective graphical models is proposed by~\cite{CGMs} as a formalism to perform inference in aggregate noisy data including ensemble flows. \cite{ApproxCGMs} studied the intractability of the exact marginal inference in CGMs, and proposed an approximate MAP estimation as a substitute. Following this success, \cite{MPCGMs} developed the non-linear belief propagation algorithm to perform approximate MAP inference in CGMs. Bethe-RDA is another algorithm dedicated to aggregate inference in CGMs via regularized dual averaging (RDA) with guaranteed convergence. Recently, \cite{Bernstein16} developed an approach of moments estimator to learn the parameters of the Markov model from aggregate noisy flows.
 
%  \cite{MOTPGM,HaaslerRCK19} recently investigated the problems of estimating ensemble flows from a graphically structured multi-marginal optimal transport perspective. In particular, \cite{MOTSBP} studied a tree-structured multi-marginal optimal transport, which allows to consider various related problems such as information fusion under a unified MOT framework. \cite{Chen01} first studied the inference (filtering) problems in CGMs based upon the tree-structured MOT framework. \cite{Chen02} derived an approximate EM algorithm to conduct learning and inference in CGMs. 
%  Nonetheless, the approximate EM scheme still admits expensive time complexity when it faces with large-scale real-world applications involving tens of thousands of states.
% To address this limitation, we are motivated to leverage the sparse network structure among the states of the Markov model, and resorts to a method of learning graph-structured transition matrix. The developed EM algorithm is appealing for large-scale settings, compared with the approximate EM algorithm~\cite{Chen02} as demonstrated in the experiments (Sec.6).

% Other related studies include neural CGMs for the inference in spatial-temporal population flows~\cite{NCGMs}. In particular, we also developed a graph neural network method to perform inference in aggregate noisy data by implicitly encoding the model parameters of the Markov model, rather than learning these model parameters explicitly via neural networks.

% % Prior works on dynamic networks modelling include the exponential random graph model (ERGM)~\cite{Guo}, matrix and tensor factorization based methods~\cite{MTF}, continuous-time diffusion models~\cite{CTDN11,CTDN12, CTDN13a, CTDN13b} and statistical models~\cite{LSM, DIRM, NBDN}. Statistical dynamic network models received considerable attention because these models have favourable interpretability by providing uncertainty estimates for the uncovered latent representations~\cite{PHoff}.
% % % \textcolor{blue}{, which makes it especially appealing to analyzing partial observed relational data and complicated multi-relational graphs data}.
% % %An amount of statistical dynamic network models have been proposed though we discuss only dynamic stochastic blockmodels (DSBMs) and dynamic latent feature relational models (DLFRMs) since they are more closed to our proposed models in terms of model constructions and properties. 
% % Dynamic extensions of the mixed membership stochastic blockmodel (MMSB)~\cite{MMSBM} have been developed~\cite{Fu09, xing2010, EMMB} using linear state space models to capture the evolution of \emph{real-valued} node class memberships. 
% % We note that a mixed memberships model can be recovered from our proposed model by the normalization of the gamma distributed memberships to restrict probabilities normalized to one because of the relationship between the Dirichlet and gamma distribution~\cite{ferguson1973}.
% % %We note that a dynamic mixed membership model can be recovered from our proposed model restricting gamma-distributed membership vector normalised to one because of the relationship between the Dirichlet and gamma distribution~\cite{}.
% % Recently, an extended Kalman filter (EKF) based algorithm~\cite{DSBM} was proposed to infer dynamic stochastic blockmodels (SBM) with competitive performance. Dynamic extensions of the latent feature relational model (LFRM)~\cite{LFRM} using an infinite factorial hidden Markov process to capture the evolution of \emph{binary} node-group memberships include the dynamic  relational  infinite  feature
% % model (DRIFT)~\cite{DRIFT}, the latent feature propagation model (LFP)~\cite{LFP}, and the dynamic multi-group membership graph model (DMMG)~\cite{MGMM}. 
% % %Recently, a novel network model based on completely random measures has been proposed~\cite{Caron} to model sparse graphs. The dynamic extension of the method of~\cite{Caron} has recently been proposed~\cite{SDN} using the dependent gamma process~\cite{Caron_dGaP} to model latent sociabilities. 
% % % Note that the method of~\cite{SDN} cannot characterize inter-group interactions among nodes in networks that exhibit stochastic equivalence~\cite{hoff_2008_nips}.

% % Our proposed model is a form of Poisson factorization model~\cite{Canny, NBP, Gopalan, Charlin, CPD}, and can be considered as the dynamic extension of the hierarchical gamma process edge partition model (HGaP-EPM)~\cite{EPM}. 
% % % However, our distinct contributions here for dynamic networks were not exploited before. 
% % % We highlight our contributions regarding to each of the two main components of the proposed model in turn. 
% % The dependent CRM framework~\cite{tCRM} has been exploited for dynamic topic models and dependent latent feature models~\cite{KBP} previously. To the best of our knowledge, this is the first attempt to model activity and inactivity of latent groups using a thinned CRMs framework in dynamic networks modelling. Our Markov chain construction, used to capture the evolution of node-group memberships, is inspired by the data augmentation technique~~\cite{NBP} that has been exploited for dynamic matrix factorization~\cite{DFM, PGDS} and deep gamma belief networks~\cite{AGBN}. We note that the dynamic gamma process Poisson factorization (D-GPPF)~\cite{DGPPF} has been proposed using gamma Markov chains to model the evolution of latent groups while the D-GPPF assumes node memberships are static over time. 
% % % However, the D-GPPG cannot model inter-group interactions among nodes. 
% % Notably, a gamma Markov chain can be alternatively constructed conditioning the state at every time step on the state at previous time step via gamma scale parameters~\cite{DEF,DCF}. 
% % %[1]
% % %T. S. Ferguson. A Bayesian analysis of some nonparametric problems.
% % %The Annals of Statistics
% % %,
% % %1(2):209?230, 1973
